The Word Problem for Braided Monoidal Categories is Unknot-Hard

We show that the word problem for braided monoidal categories is at least as hard as the unknotting problem. As a corollary, so is the word problem for Gray categories. We conjecture that the word problem for Gray categories is decidable.

==> eptcsdata.tex <==
\providecommand{\firstpage}{72}
\providecommand{\publicationstatus}{K. Kishida (Ed.): Fourth International Conference\\
on Applied Category Theory (ACT 2021).\\
EPTCS 372, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.372.6}{10.4204/EPTCS.372.6}}

